Remembering George Smoot

George Smoot (1945-2025) was a major figure in observational cosmology, particularly through his role in the precision measurement of the CMB dipole and the discovery of the primordial CMB temperature anisotropy as part of the COBE team. This collection of 33 essays from collaborators, colleagues, students, and friends offers varied insights into the work, career, and life of George Smoot.

==> broadhurst.tex <==


\phantom{tom} 

\begin{figure}[h] 
\begin{center}
\includegraphics[width=0.7\textwidth]{%
georgeAndBroadhurst.png}
\end{center}
\caption{%
\textbf{George and Tom Broadhurst at the IAS HKUST.}
[Photo credit: N\'ora Csisz\'ar]
}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{%
georgeDIPC.jpg}
\end{center}
\caption{%
\textbf{At DPIC, Euskadi (Pa\'\i s Vasco).}
(From left to right): Tom Broadhurst, Thomas Frederiksen, Pedro Miguel Echenique Landiribar, George Smoot, Ricardo Diez Muñoz, and Fernando Cossio.
[Photo credit: N\'ora Csisz\'ar]
}
\end{figure}


Working closely with George over the past eight years has been a special and fruitful time for me and our 
shared research students, initially at the Hong Kong Institute for Advanced Study (IAS), 
where I was fortunate enough to be invited for 
long visits by the visionary director Henry Tye. % a founder of inflationary cosmology.  
George's office in Hong Kong was 
really interesting. Several of his patented inventions could be tried out, including an oscillating pink 
toning cushion, a wave motion bed for curing jet lag, and an air purifier displaying the pollutant spectrum, all 
for sale on the mainland. As a special treat George might offer a chocolate Nobel medal.

Previously we had known each other only a little in Berkeley, where I suffered as a junior lecturer in the 
mid-90s, occasionally managing to escape the pressure of campus for a lunch with George and his fun team on the 
terrace at LBL overlooking the San Francisco Bay, where he enjoyed teasing me and the English. Two decades then passed before 
reconnecting properly at the IAS when both of us had more time. Lunch became the major daily focus, 
together with Henry Tye and George's %youthful Hungarian 
partner N\'ora, who also enjoyed a good laugh, often about 
George, about which he was very sporting. Conversation often turned to the serious subject of the uncertain 
future, about which George actually had a stake in shaping, with his supercooled quantum detectors at the IAS 
lab, and rocket ideas, where he could really get into details about 
%engine EMF.  
electric propulsion. 
These were great times, with 
whiteboards covered, grants won, and students joining in, before Covid and the crackdown arrived from the 
mainland, with research more focused on surveillance technology. Fortunately, with George we could continue our 
work in Spain at the 
Donostia International Physics Center (DIPC) near my home, with more excellent lunches in San Sebasti\'an thanks to the generous 
and visionary directors of the DIPC, who also enjoyed George's humour and a shared interest in quantum computing.

Over the past eight years my research with George has really blossomed. With his keen eye for data and strong 
background in general relativity,
we became pretty convinced that 80\% of the high chirp mass LIGO events are highly magnified at 
cosmological distances. We also explored light axions as the dark matter, as large waves, together with our 
students making definitive predictions, the last of which used ``smooth'' dark matter to explain the 
predominance of elongated galaxies uncovered by JWST (James Webb Space Telescope). This was published in \textit{Nature} last year, marking a fitting 
end of a special era, before we suddenly lost our talented and kind-hearted friend, the legendary George.



==> johnBerliner.tex <==

\phantom{carnitas} 

\begin{figure*}[h]
\begin{center}
\includegraphics[width=0.45\textwidth]{%
carnitasOne.jpg}
\end{center}
\caption{%
\textbf{George Smoot and John Berliner at the Los Michoacanos in Cabo.}
[Photo credit: N\'ora Csisz\'ar]
}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=0.7\textwidth]{%
carnitas2.jpg}
\end{center}
\caption{%
\textbf{George Smoot and John Berliner enjoying carnitas in Cabo.}
[Photo credit: N\'ora Csisz\'ar]
}
\end{figure*}

I first met George Smoot twenty-five plus years ago in Cabo San Lucas, Mexico.
George was definitely a foodie and relished finding off-the-grid restaurants. 
His favorites immediately became a traditional must go on a consistent basis.

Here was a man of such knowledge and intellect. Yet during our weekly visits to Restaurante Carnitas Michoacán, 
he always blurted out with child like excitement, ``Carnitas, Carnitas'' each and every time.
He (me too) also enjoyed eating at home, at ``Chez N\'ora,'' kindly referring to his partner N\'ora, who always and consistently
prepared tasty and healthy meals at their beachfront property in Cabo. 

George had an interesting and delightful sense of humor, as well as sharing in his many interesting 
projects and his prospective thoughts on world events.
He was so appreciative of his experiences in Cabo, the community and the friendliness of the Mexican 
people, that he made it a point to  give back.
George decided years ago to share his knowledge in cosmology, physics, science, 
and more throughout Mexico, delivering speeches to  academics as well as to anyone 
else interested in attending. This included the city of La Paz, the state capital 
of Baja California Sur. Its proximity to Cabo allowed professors, students, and others 
living in Cabo also to attend.

This reminds me of another fond memory.
Our weekly trips to Costco-Cabo for hot dogs and a slice of pizza followed by shopping was
also one of George’s pleasures. Of course just like Carnitas, Costco was once a week and on a specific day.
Multiple times on a Costco trip, my dear friend was approached by ``fans'' asking for selfies and 
to share their delight in meeting him. This included adults and youngsters new to cosmology.

I am extremely grateful that I was given the gift of George’s friendship.
Time spent together in Cabo San Lucas, Paris, and our excursion side trips were very special.
Multiple trips with my wife Angelica, with accommodation provided by George and N\'ora at their 
fabulous apartment, as they always wanted to make sure that we had a good time in Paris.
My last trip to Paris was in August 2025 with my daughter, two granddaughters, and a pre-born (born in December 2025)
granddaughter. We took a trip to Paris Disney, and the excitement of 10-year-old and  12-year old young girls was almost outdone 
by the enthusiasm and exuberance that George and N\'ora expressed in the ``Le Royaume Magique,'' especially N\'ora, 
but George could not help but smile and laugh all the way to the castle!

My love, care, and respect for George continuously expanded throughout our friendship.
I cherish all the memories he left behind.

Thank you George. 

%John Berliner

\clearpage 


==> linder.tex <==

The first time I met George person to person was when I attended his
revelation (word advisedly chosen!) of the discovery of
the 
Cosmic Microwave Background (CMB) fluctuations at the 1992 American Physical Society meeting. 
I was struck by not just the incredible scientific result but the flair with
which it was presented. I hung around afterward and George was kind enough
to give me an advance copy of the paper. The next time I had the chance to
sit down with George was when I interviewed for a position at 
Lawrence Berkeley Laboratory (LBL). George
put me at ease and turned it from an exam into a collegial discussion of what
new science opportunities we could develop. 

George strongly defended quality and innovation to help grow LBL, arguing for
example that prize fellows should be not just whom the Physics Division
needed that year but people who would break new ground and bring new
capabilities. This philosophy carried
forward when he established the Berkeley Center for Cosmological Physics (BCCP),
with each year bringing an energetic group of postdocs and a tangible
atmosphere of brainstorming, initiative, and collaboration.
George also always reached out to other groups internationally, for example
strongly supporting a group of Mexican institutions in forming their
national and very successful Instituto Avanzado de Cosmolog\'\i a (IAC). This later
gave rise to the infamous Cosmology on the Beach (more formally known as
Essential Cosmology for the Next Generation) winter schools in Mexico,
which is into its second decade in training many generations of students
from the US, Mexico, and around the world.

One of my clearest memories of George from one of these schools 
brings together several aspects of George's personality. He was to give
a public lecture to school children as part of the conference, set outdoors
near the Mayan ruins of Tulum. It was quite windy and it took a long time
to set up. The free-standing projection screen kept blowing down.
George showed incredible patience throughout and ended up giving the
talk much appreciated by the
school children while helpers held the edges of the screen. At the same
meeting, George brought Mickey Hart, former drummer from the Grateful
Dead, to premiere his ``Rhythms of the Universe,'' turning astronomical
data into sound and percussion. These aspects of reaching out to teach,
to communicate between areas---and to eat great food---as well as advancing
our knowledge of the universe were all George. 



==> lineweaverV3.tex <==
%Remembering George Smoot  
%by Charley Lineweaver

\phantom{Raul} 


\begin{figure*}[h] 
\begin{center}
\includegraphics[width=0.9\textwidth ]%
{lineweaverFigOne.jpg}
%lineweaverFig2.png
%-rw-r--r--@  1 mabucher  staff     36227 22 mar 19:27 lineweaverFig3.jpg
%IMAGE PLACEHOLDER
\end{center}
\caption{%Figure 1. 
\textbf{LBL/DMR Smoot group photo (May 1992).}  Left to right: 
Luis Tenorio, Charles Lineweaver, John Gibson, Giovanni 
De Amici, George Smoot, and Jon Aymon. George had this semi-disassembled radiometer hauled out of the Smoot group's 
scrap heap for the photographer. It had been used in the late 1970s to measure the dipole in the CMB.  It was a 
nostalgic moment for George and Smoot group veterans John and Jon. And for Luis and me this was the closest we ever 
came to the hardware whose data we had been analyzing every day for the previous two years.
[Photo courtesy of Charley Lineweaver]%
}
\end{figure*}

On 26 September 2025, I received an email telling me George had died. I looked out the window. Branches of a 
eucalyptus tree were dancing in small gusts of wind\ldots George\ldots George was my PhD supervisor at Berkeley from 1990 to 
1994, more than 30 years ago.  My life with George began in 1990 after I had passed my qualification exams and was 
looking for a PhD research topic. I noticed a small poster in Burgess Hall advertising a position up at Lawrence 
Berkeley Laboratory (LBL) to help analyze data from the Differential Microwave Radiometers (DMR) that had just been 
successfully launched (18 November 1989) on NASA's COBE satellite. It sounded like the greatest job I had ever heard 
of---cosmology and the thrill of finding out something new about the entire universe. The next day I took the campus 
bus up the hill to LBL to introduce myself.  George seemed amiable and outgoing---like a confident extroverted geek 
who liked to joke around.  He didn't seem very concerned about my qualifications. Maybe I was the first (or maybe the 
only?) grad student to respond to the advertisement.  Or maybe just being a Berkeley physics grad student was good 
enough. George seemed so welcoming that it wasn't clear to me who was interviewing whom.  He invited me to have lunch 
at the LBL cafeteria with a couple of members of his team. We talked about the COBE mission, the cosmic microwave 
background, and Hubble's Law.  I let him know that I was taking Joe Silk's cosmology course. And to show him that I 
knew something about cosmology, I started explaining
%holding forth on 
Hubble's law and how it was consistent with the expansion of 
space, not with some kind of explosion. George interrupted me, ``Maybe the Big Bang was an explosion.''  He scribbled on 
a napkin. ``An explosion would produce the same velocity-distance relationship---debris scattered with the highest 
velocity would be the furthest away.'' I stopped chewing and looked down at the tiny galaxies exploding away from the 
center of the napkin. ``But we'd have to be at the center,'' I objected and looked for his response. He made an almost 
imperceptible nod as if he didn't want to let me know what he thought. He seemed unimpressed at my conventional 
response, but at the same time his nod said, ``OK, you can join the team." Thus began my initiation into George's 
world.

After this lunch Jon Aymon (see Figure), who took care of the computing needs of the Smoot group, set me up with a 
chair and a small desk with a large computer monitor. He gave me a computer account and showed me where to find a set 
of thick, cheap, orange-vinyl Fortran 77 computer manuals that were soon to become my nemesis. My desk was next to 
Luis's, a Berkeley grad student in math from Mexico. Thus began my life as a DMR data analyst writing Fortran programs and 
making plots with IDL. The first year was challenging because I knew neither Fortran nor IDL. I had never coded before. 
I had never used a computer (remember this was early 1990). I had never made a plot.  Why in the world did he accept 
me for this job? Maybe he had scared away other students. Office scuttlebutt suggested that George could be hard to 
work with. This was true. But the many years I had spent in locker rooms gave me a thick skin and a healthy immunity 
to playful derision.

George was my PhD supervisor from 1990 to 1994.  During those four years we spent hundreds of hours analyzing data 
from the COBE DMR.  I made hundreds of plots and then explained what I had done. He 
pointed out potential problems with what I had done. We argued. He was right most of the time. Then we tried to figure 
out ways to improve and extend the analysis. Usually we came up with several alternatives. If we couldn't figure out 
which way to do the analysis, George inevitably recommended all of them.  It was my job for the rest of the night to 
explore the alternatives for discussion the next day.

In the Smoot group, George usually expected more from us than we could do.  He would come into my office several times a 
day to remind me of what he had asked me to do earlier.  He often seemed disappointed in the progress I had made 
since our last meeting 30 minutes ago.  In 
\textit{Wrinkles in Time} (p.~143) George described how his early U-2 dipole results 
had been subject to similarly severe criticism:
\begin{quote}
I don't fault them for their caution. They were doing to us what Luis Alvarez always did to us, his students, when 
we claimed to have detected this or that effect. He grilled us, often brutally, to ensure we had dotted every `i' and 
crossed every `t.' In science such grilling is essential.
\end{quote}

Thus, in being hard on us George was passing on the important lessons he had learned from his mentor Luis Alvarez.  
But luckily, we were not defenseless.  A senior postdoc Al Kogut had learned a bit about George's backstory and had 
come up with an interesting technique to deal with George. George had come to Berkeley in 1970 (see Figure).  In 
1978 after 19 years of work, a math PhD student at nearby Stanford University had been told that he would not be 
getting a PhD. In frustration he had murdered his PhD supervisor with a ballpeen hammer. This must have made a deep 
impression on George, because in desperation and as a joke, whenever George had overstayed his welcome in Al's office, 
Al would quietly open up the drawer of his desk, take out a ballpeen hammer and slowly start tapping it on his knee. 
George would quietly and almost apologetically beat a retreat.

George liked to laugh. He had a clever, mischievous, often puerile sense of humor with an outsized capacity for 
derision. But when it became too belittling, I belittled him back. And to his credit, he laughed at himself, knowing 
(I think) that he deserved it.

George was a hard-working, theoretically-savvy observational cosmologist. But with grad students and postdocs he was 
not known for diplomacy.  Most of George's joking was his way of trying to get us to work harder. He came to work 
early, left late, and worked every weekend.  He was a workaholic who was harder on himself than he was on us. Science 
and the thrill of finding out something new about the universe was more important to him than his personal life. 
George had no wife nor children.  Everything was to be sacrificed at the altar of knowledge. In his Nobel Prize biography,
George wrote about his first exposure as a child to university education: ``The seriousness of learning was tempered 
with fun, so it was a wonderful place to be.''  I'm sure he was trying to duplicate this early experience and make the 
Smoot group a ``wonderful place to be.'' In many ways it was.

\begin{figure*}
\begin{center}
\includegraphics[width=0.99\textwidth ]%{nyt_george_photo2.png}
{lineweaverFig2.jpg}
%IMAGE PLACEHOLDER
\end{center}
\caption{%
%Figure 2. 
\textbf{Stages in the life of George.}
[Image courtesy of Charley Lineweaver]}%
\end{figure*}

George's relentless work ethic and uncompromising determination probably came from his educationally rich but 
financially modest upbringing. His Nobel Prize biography explains how after long hours of reading during the Alaskan 
winters, he read himself into thick glasses by age 10. ``My father drilled me in the basement, force-feeding 
trigonometry and introductory calculus, courses that were not given at my high school.''

Poor George! He worked so hard and expected so much of himself. No wonder he expected so much of us.  He strongly 
believed one needed to work hard to achieve anything.  He thought that people who had made something of themselves 
deserved their honors. The less appealing corollary was that if you didn't achieve anything, it was on you.  Laziness 
and apathy were so far from George's personality traits that he couldn't understand them. He was no dour Thomas 
Gradgrind, but in my struggles to deal with George, I sometimes asked myself, ``Is he a social Darwinist?''  During the 
hundreds of hours we talked, religion never came up, so I don't know what his religious views were.

George had a vast supply of idiotic and brilliant ideas.  Occasionally, I would ask George about some weird 
semi-philosophic idea like: Where did the rest frame of the universe (the CMB rest frame) come from? Was it somehow 
chosen from a larger distribution of possibilities? Was the CMB dipole only due to our velocity? George's response to 
these queries was usually, ``Yeah, yeah.'' (I've already thought of that.) Several times when I challenged him on his 
hubris, he walked over to his file cabinet and dug out a five-year-old half-finished draft of a paper on pretty much the 
same topic.

I spent much of the summers of 1990 and 1991 at the Cosmology Data Analysis Center (CDAC) in hot and humid Greenbelt, 
Maryland. George owned a McMansion nearby. At the CDAC, Luis Tenorio and I got to know the other members of the DMR 
team.  George got up early every morning, ate his cereal with a banana, and was gone before I got up. On the kitchen 
counter he usually left a copy of Atlantic magazine, which he had perused over breakfast.  He had a subscription. After a 
year of working with DMR data, one day in the halls of the CDAC, George approached me with an almost ritual solemnity: 
``What do you want to work on?'' he asked, pronouncing each word carefully.
%
His voice had an unusual, ceremonial dignity. I had never heard him speak to me with such commitment. As my 
supervisor, he felt it was his sworn duty to help me become a scientist. Apparently it was my time. ``The dipole. I 
want to write a paper on the DMR dipole,'' I responded confidently. He listened, considered, and then approved of my 
decision with a nod of acceptance. Unfortunately, early the next day Al Kogut had produced a draft of a dipole paper 
with his name first. Mine was second.  I was disappointed for a few weeks, but when Al expertly converted my ten-page 
summary of the dipole literature into two \textit{Astrophysical Journal} paragraphs, I had to accept that at this point I wasn't ready to be lead 
author. This lucky setback several months later led to my research focusing on the correlation function analysis of 
the DMR maps.

In \textit{Wrinkles in Time} 
(with Keay Davidson, p.~279), George described our collaboration in early 1992, a few months before 
we announced our discovery of fluctuations in the cosmic microwave background as follows:
\begin{quote}
Another day passed, and Charley was 
still distracted by his idea for improving the program. He still hadn't subtracted the quadrupole from the map. I 
could bear it no longer. About midnight I went across the hall to where he was working and said, ``Don't go home until 
you run the maps through your program with the mean, the dipole, and the quadrupole subtracted.'' I made it sound 
urgent, but didn't say why, and then left for home. About three hours later, the run completed, Charley slipped some 
plots under my office door \ldots ``Here are the plots you asked for, Eureka?''
\end{quote}

What's funny about this story is that he had told me something similar almost every night for the previous two weeks. 
In fact, I had slipped late-night plots under his door virtually every night for the previous year. But in Spring 
1992 things were coming to a head. It was only that night that I had written ``Eureka.''  Here is how George 
described the same scene twelve years later in his Nobel Prize Biography:
\begin{quote}
The observed quadrupole was lower than anticipated compared to the higher order fluctuations (having smaller angular 
scales). Finally, removing the quadrupole effect from the data, I found that the observed fluctuations fit predictions 
for a scale invariant spectrum. To confirm this finding, I suggested to graduate student Charles Lineweaver to look at 
the data with the quadrupole removed, without telling him what he would find. He used a different version of the 
analysis program that he had written rather than the one I wrote. When Lineweaver left the office in the early morning 
hours, he slipped his results under my office door with the message: ``Here are the plots you asked for. Eureka?'' They 
agreed precisely with my own calculations. Everything had fallen into place.
\end{quote}

When I read George's above words ``without telling him what he would find,'' I was reminded of a joke George had told 
me in my first year as the only grad student he was supervising:

``How are grad students like mushrooms?''

``You have to keep them in the dark and feed'em shit.''  

My reply was something like, ``Very funny George. You do know that I'm your grad student?''

My version of the ``Eureka?'' story starts a bit earlier. Luis and I wrote code, but we also had to document it to make 
it part of the validated DMR pipeline. This documentation sometimes took as long to write as the code itself. Official 
DMR standards had to be maintained.  At the same time Ned Wright (and apparently George) were writing their own 
private, no-documentation-necessary code to analyze the data in similar ways.  Late in 1991 my program could make a 
variety of galactic plane cuts, efficiently remove the best-fit dipoles, and then compute the correlation function of 
the resulting DMR sky maps.  I was proud of what it could do, but when George came back from a COBE Science Working 
Group meeting in Washington in late 1991, he wasn't impressed. (I'm not sure my coding skills ever impressed George.)

``Try taking out the best-fit quadrupole,'' he said.

``But we're looking for the quadrupole,'' I said. 

``Just take out the quadrupole,'' he repeated.  

``That'll remove some of the signal we're looking for.''

``Just take out the quadrupole,'' he said with some annoyance.  

``OK, but with the cuts, it's not orthogonal to the dipole and octopole.''  I wasn't telling him anything he didn't know.

``Just take out the quadrupole,'' he said and walked back to his office.  

Removing the quadrupole was an interesting request. Detecting the quadrupole was one of the most important goals of 
the DMR, so removing it seemed like throwing out the baby with the bathwater.  On the other hand, our main enemy, the  
galactic foreground, was predominantly a quadrupole, so it made sense to remove it in the hope that the higher order 
(smaller scale) power in the map would become more obvious in the correlation function plots that I was making, (e.g., 
Fig.~2 of Smoot et al.~1992).  We had been ``removing'' the galaxy by the crude but easy method of making galactic plane 
cuts at $10^\circ ,$
$20^\circ ,$ $30^\circ ,$ and $40^\circ $ above and below the galactic plane.  At Goddard, Gary Hinshaw and Chuck Bennett 
were working on making maps of galactic emission (synchrotron, free-free, and dust). It took me a while to remove the 
quadrupole. But in my defense, subtracting the best-fitting quadrupole from sky maps out of which various galactic 
cuts had been made, was not straightforward.  Removing  $30^\circ $ left you with only half the sky---two separate polar 
caps each 1/4 of the sky. After such large galactic cuts, the dipole and quadrupole were no longer orthogonal.  Power 
would spread out and leak into the other multipoles. Yikes! And soon it wasn't only the quadrupole I had to subtract.  
Gary Hinshaw sent me the latest models of the galactic foreground, which could also to be subtracted before computing the 
correlation function. The ``Eureka?'' moment George was describing had come because the signal we were seeing in the 
maps was still there after the galactic cuts. It was still there after the maps of galactic emission had been removed. 
It was still there after I had removed the best-fitting quadrupoles. And it was still there after making all possible 
combinations of the above.  We had found the long sought after seeds of large scale structure.

In early 1992, there was a Science Working Group meeting at Nancy Boggess' house. I was there with another grad 
student Ken Ganga. We were relegated to the basement to play pool while upstairs George tried to convince the Science 
Working Group, huddled together in a secret cabal, that we had indeed found fluctuations in the CMB. This was when the 
final decision to publish the data was made. I suspect that as usual, the moderating influence and wisdom of Rai Weiss (another 
Nobel Prize winner) had made the decision go more smoothly. 
%If one were to compare the Science Working Group to Star 
%Wars characters, Rai Weiss was Yoda, Ned Wright was Hans Solo, John Mather was Luke Skywalker while George was Darth 
%Vader.

\begin{figure*}
\begin{center}
\includegraphics[width=0.7\textwidth ]%
{lineweaverFig3.jpg}
\end{center}
\caption{%Figure 3. 
\textbf{Our photographic re-enactment of the Eureka? moment for People magazine on 5 May, 1992.}
I'm standing, George 
is seated. 
The after-midnight plots George was referring to were Figures 2 and 3 of our 
discovery paper (Smoot et al.~1992). In this photo, George is holding a version of Figure 3 of Smoot et al. 1992. 
George's expression has an unusual deference, almost as if he is asking my approval. My desk today looks just like 
his did.
[Photo credit: John Storey. Courtesy of Charley Lineweaver]}%
\end{figure*} 

It is unfair to the DMR team to focus on this ``Eureka?'' moment.  The press and the public's desire for a simplistic 
``Eureka'' has been problematic since Archimedes, and is maintained by the prohibition of awarding the Nobel Prize to 
groups.  Our discovery was the product of a steady plod during which our confidence slowly grew. George writes, ``I was 
obsessed with detecting possible causes of error.'' Yes, he was. And so was the entire DMR team.  Almost every day of 
the previous year had been a steady hunt for elusive systematic errors that could mask or mimic the signal we were 
looking for.  The monstrously detailed, thankless-but-necessary write-up of this hunt was led by the imperturbable Al 
Kogut (Kogut et al. 1992), heavily prodded on by George.


\begin{figure*}
\begin{center}
\includegraphics[width=0.7\textwidth ]%{nyt_george_photo2.png}
%RAUL
{lineweaverFig4.png}
\end{center}
\caption{%Figure 4. 
\textbf{%
George presents our results, April 23, 1992, at a meeting of the American Physical Society (APS) in 
Washington, D.C.}  
Our results and his statement ``if you're religious, it's like seeing God'' touched off a media 
frenzy rarely seen at scientific conferences.
[Courtesy of Charley Lineweaver]}
\end{figure*}

Stephen Hawking called our discovery the ``scientific discovery of the century, if not of all time.'' This Hawking quote 
is easily dismissed as sensationalism.  But there is science behind Hawking's praise. The fluctuations we had found 
were at scales larger than a few degrees---too big to be causally connected. In the standard Big Bang model (without 
inflation), the opposite sides of a large spot in the DMR map could never have been in causal contact, and so could not be 
part of the same structure. And yet there they were.

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.7\textwidth ]%
%{lineweaverFig5.png}
%\end{center}
%\caption{Figure 5. George the geeky adventurer performing for the People Magazine 
%photographer in May 1992. George was usually 
%game for any mischievous fun. Roller blading was not one of his hobbies. Who pulls 
%up their shorts that far and tucks 
%in their shirt like that?}
%\end{figure*}

George appeared twice on the television show ``Big Bang Theory,'' as well as the quiz show 
``Are You Smarter than a 5th Grader?''  I'm convinced that his playful childishness---some 
would say ``emotional immaturity''---contributed to his many scientific insights. One of the most 
important unchildish lessons I learned from George was about error bars. Compared to the work it 
takes to get a good estimate, you need to invest about ten times longer to figure out what the 
error bars on that estimate are.  I have passed this seemingly depressing wisdom on to all my students, 
who are themselves passing it on as we speak.

As I was finishing up my PhD, George began to teach an undergraduate physics course at Berkeley. This was a new 
experience he seemed to enjoy. One day before I left for a postdoc in Strasbourg, I asked him what he was going to 
teach that day. ``The three laws of electromagnetism,'' he said. ``Which are?'' I asked. 
``Don't you know the three laws of electromagnetism? I= V/R, IR =V, and R=V/I.'' 
He laughed and enjoyed how long it took me to get the joke. ``Very funny 
George.''

\begin{figure*}
\begin{center}
\includegraphics[width=0.7\textwidth ]%
{lineweaverFig6.jpg}
\end{center}
\caption{%Figure 5. 
\textbf{The Cosmic Microwave Background from Space.}
COBE and the follow-up CMB space missions WMAP and Planck gave increasingly precise characterizations
of the CMB temperature anisotropies at ever greater angular resolution and sensitivity.
Today the initial conditions of the universe have been precisely characterized by observation. 
[Credit: COBE Collaboration/NASA \copyright USG]
}
\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.7\textwidth ]%
%{lineweaverFig7.png}
%\end{center}
%\caption{Caption.}
%\end{figure*}

%\begin{verbatim}
%Figure 6 
%The Legacy of George Smoot and CMB maps.
%Date, Project, angular resolution, number of frequencies
%
%1992	 NASA COBE DMR 	7 degrees 	3
%2003 	    NASA WMAP   	0.2 degrees	5
%2013 	     ESA Planck 		0.1 degrees  	9
%\end{verbatim}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.7\textwidth ]{nyt_george_photo2.png}
%\end{center}
%\caption{%
%%A black-and-white photo of a youngish George Smoot, wearing glasses, a button-down shirt and tie and dark trousers,
%%standing in front of a transparent globe.
%Dr. Smoot in 1992, the year he announced findings that helped transform
%cosmology from a field largely based in speculation to a science grounded in precise measurement. [Credit: Susan Spann]}
%\end{figure*}
%Someone needs to overcome the egos of the principal investigators and make all three of these maps with the same color 
%scheme. www.forbes.com/sites/startswithabang/2018/07/19/how-the-planck-satellite-changed-our-view-of-the-universe/ 


\begin{table}
\begin{center}
\begin{tabular}{| c | l | c |  c |}
\hline 
Date & Experiment & Angular Resolution & Frequency Channels \\
\hline 
1992 & NASA COBE DMR & $7^\circ $ & 3 \\
2003 & NASA WMAP     & $0.2^\circ $ & 5 \\
2013 & ESA Planck    & $0.1^\circ $ & 9 \\
\hline 
\end{tabular}
\end{center}
\caption{\textbf{COBE and its Successor CMB Space Missions.}}
\label{cmbSpaceTable}
\end{table}

The COBE DMR experiment was the first in a highly successful campaign to map out the CMB anisotropies
in temperature, and later in polarization, at ever greater precision, and thus establish the initial conditions 
of the universe. The Figure and Table \ref{cmbSpaceTable} compare the COBE DMR with the two follow up dedicated
CMB space missions WMAP and Planck. This is not the whole story, 
%in additional to space-based observations observations from the ground also 
because ground-based observations on even smaller scales 
played a key role.\footnote{See https://lambda.gsfc.nasa.gov/product/expt/ for
a compilation of the many CMB experiments over the years.} %It was exciting to be part of this adventure.
In a ``Closer to Truth'' interview with Robert Kuhn,\footnote{www.youtube.com/watch?v=S2jnk3ZfUME} 
George explains the meaning of CMB maps. ``When you look at this map, you're simultaneously seeing what was once the 
smallest thing in the universe 
and is now the largest things in the universe. So it's really cool. It's way cool...The universe is a giant 
microscope.''

In their \textit{Nature} 
obituary of George, Doug Scott, Joe Silk, and Tom Broadhurst wrote, ``George was always interesting and 
fun to be with \ldots He was a strong personality who pursued answers to some of the biggest questions in science.'' Yes, 
very true. They also called George ``charismatic.'' That seemed like a funny word. But I could understand why they 
wrote that. Searching for better words to describe his effect on me, I came across George's description of his mentor 
Luis Alvarez. It seems just as appropriate as a description of George's own legacy 
(\textit{Wrinkles in Time}, p.~90):  
\begin{quote}
To all 
of us, Luis was both an inspiration and a source of some terror\ldots He was one of the most diverse, ornery, and 
brilliant humans one could meet, and inexorably had a major influence on our careers and our ideas of how to do 
scientific research.
\end{quote}

\begin{figure*}[h] 
\begin{center}
\includegraphics[width=0.7\textwidth]{%
b50roof.jpg}
\end{center}
\caption{%
\textbf{George and colleagues on LBL Building 50 roof.} 
(left to right) Giovanni de Amici, Charles Lineweaver (kneeling), Luis Tenorio, George Smoot (bending), John Gibson (in back), and Jon Aymon.
[Photo courtesy of Lawrence Berkeley National Laboratory]
}
\end{figure*}



